A Crevice on the Crane Beach: Finite-Degree Predicates

First-order logic (FO) over words is shown to be equiexpressive with FO equipped with a restricted set of numerical predicates, namely the order, a binary predicate MSB$_0$, and the finite-degree predicates: FO[Arb] = FO[<, MSB$_0$, Fin]. The Crane Beach Property (CBP), introduced more than a decade ago, is true of a logic if all the expressible languages admitting a neutral letter are regular. Although it is known that FO[Arb] does not have the CBP, it is shown here that the (strong form of the) CBP holds for both FO[<, Fin] and FO[<, MSB$_0$]. Thus FO[<, Fin] exhibits a form of locality and the CBP, and can still express a wide variety of languages, while being one simple predicate away from the expressive power of FO[Arb]. The counting ability of FO[<, Fin] is studied as an application.

==> define.tex <==
\makeatletter

\def\defmath#1#2{\protected\def#1{\ensuremath{#2}\xspace}}
\def\defmathtext#1#2{%
  \edef\@@star{\csname\expandafter\@gobble\string#1 star\endcsname}
  \edef\@@nostar{\csname\expandafter\@gobble\string#1 nostar\endcsname}
  \expandafter\def\@@nostar{\text{\normalfont#2}\egroup\xspace}%
  \expandafter\def\@@star{\text{#2}\egroup\xspace}%
  \protected@edef#1{%
    \noexpand\bgroup%
    \noexpand\protect\noexpand\@ifstar%
    \unexpanded\expandafter{\@@star}
    \unexpanded\expandafter{\@@nostar}}
}

\defmathtext\MSBz{MSB$_0$}
\defmathtext\ACz{AC$^0$}

%% Mathcal should be bold on a bold context.
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
\let\@mathcal=\mathcal
\def\@bfseries{bx}
\def\mathcal#1{%
  \ifx\f@series\@bfseries%
  \mathbfcal{#1}%
  \else%
  \@mathcal{#1}%
  \fi}

\def\deflogic#1#2{%
  \gdef#1##1##2]{\if##1*%
    {\def\normalfont{}%
      \mbox{\ensuremath{\text{#2}##2]}}}%
    \else%
    \mbox{\normalfont\ensuremath{\text{#2}[##2]}}%
    \fi}
}

\deflogic\FO{FO}
\deflogic\FOMOD{FO+MOD}
\deflogic\FOMAJ{FO+MAJ}
\deflogic\MSO{MSO}
\deflogic\MAJ{MAJ}
\deflogic\MOD{MOD}

\defmathtext\Maj{Maj\;}
\defmathtext\BIT{Bit}

\defmathtext\parity{\textit{Parity}}


\defmath\binal{\{0, 1\}}
\defmath\calN{\mathcal{N}}
\defmath\calC{\mathcal{C}}
\defmath\calS{\mathcal{S}}
\defmath\bbn{\mathbb{N}}
\def\lt#1{\mathbf{#1}}
\def\resp{resp.\ }
\def\lcut{\mathcal{L}}%\mathsf{cut}}
\def\rcut{\mathcal{R}}%\mathsf{cut}}
\def\bounds{\mathsf{bounds}}
\def\phi{\varphi}
\def\eps{\varepsilon}

\defmath\fin{\text{$\mathcal{F}$\kern-.1em\scalebox{.6}{$\mathcal{IN}$}}}
\defmath\arb{\text{$\mathcal{A}$\kern-.02em\scalebox{.6}{$\mathcal{RB}$}}}
\defmath\mon{\text{$\mathcal{M}$\kern-.05em\scalebox{.6}{$\mathcal{ON}$}}}
\defmath\arbu{\arb^{\text{u}}}
\def\ty{\mathsf{Ty}}

\def\foralla{\forall^\textsf{A}}
\def\foralln{\forall^\textsf{N}}
\def\forallb{\forall^\textsf{B}}
\def\existsa{\exists^\textsf{A}}
\def\existsn{\exists^\textsf{N}}
\def\existsb{\exists^\textsf{B}}

%% Predicates
\def\pr#1{\text{\ensuremath{#1}}}


%% Draft related
\def\revisionset! #1 !{\gdef\therevision{#1}}
\def\revision$LastChangedRevision:#1${\revisionset!#1!}

\def\ifzero#1{%
    \@ifnextchar{0}%
      {\expandafter\@firstoftwo\remove@to@nnil}%
      {\expandafter\@secondoftwo\remove@to@nnil}%
        #1\@nnil
}

\newif\ifdraft
\ifzero{\the\overfullrule}{\global\drafttrue}{\global\draftfalse}

\AtBeginDocument{%
  \ifdraft%
    \let\@@title=\@title
    \gdef\@title{%
      \begin{tikzpicture}
        \useasboundingbox (0, 0) rectangle (0,0);
        \node at (0, 1cm) {\small rev: \therevision, comp: \today, \currenttime};
      \end{tikzpicture}%
      \@@title}
    %\titlerunning{\@@title}%
  \fi
}

%% Theorems.
\theoremstyle{plain}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{fact}{Fact}
\newtheorem{corollary}{Corollary}
\newtheorem*{assumption}{Assumption}


\theoremstyle{definition}
\newtheorem{definition}{Definition}


\theoremstyle{remark}
\newtheorem*{remark}{Remark}

%% Qed twist
\def\addtoqedsymbol#1{%
  \let\@qedsymbol=\qedsymbol
  \def\qedsymbol{\@qedsymbol~\emph{of #1.}}}

\usepackage[e]{esvect}
\let\vec=\vv

\makeatother

